All-atom Diffusion Transformers: Unified generative modelling of molecules and materials

Diffusion models are the standard toolkit for generative modelling of 3D atomic systems. However, for different types of atomic systems -- such as molecules and materials -- the generative processes are usually highly specific to the target system despite the underlying physics being the same. We introduce the All-atom Diffusion Transformer (ADiT), a unified latent diffusion framework for jointly generating both periodic materials and non-periodic molecular systems using the same model: (1) An autoencoder maps a unified, all-atom representations of molecules and materials to a shared latent embedding space; and (2) A diffusion model is trained to generate new latent embeddings that the autoencoder can decode to sample new molecules or materials. Experiments on MP20, QM9 and GEOM-DRUGS datasets demonstrate that jointly trained ADiT generates realistic and valid molecules as well as materials, obtaining state-of-the-art results on par with molecule and crystal-specific models. ADiT uses standard Transformers with minimal inductive biases for both the autoencoder and diffusion model, resulting in significant speedups during training and inference compared to equivariant diffusion models. Scaling ADiT up to half a billion parameters predictably improves performance, representing a step towards broadly generalizable foundation models for generative chemistry. Open source code: https://github.com/facebookresearch/all-atom-diffusion-transformer

==> editing_commands.tex <==
% NOTE:
% All editing commands contain curly braces {} around them so that 
% they can easily be searched for in the final document via cmd + f.

% Highlighted comments for authors
\usepackage{soul, color}
\newcommand{\Note}[1]{}
\renewcommand{\Note}[1]{#1}  % comment out this re-definition to suppress all Notes
\newcommand{\NoteSigned}[3]{{\textcolor{#2}{\Note{\textbf{[#1: #3]}}}}}
% Alternative with highlighter color rather than text colour
%\renewcommand{\NoteSigned}[3]{{\sethlcolor{#2}\Note{\hl{#1: #3}}}}

% Specific author comments
\newcommand{\pl}[1]{\NoteSigned{PL}{blue}{#1}}  % use for notes from Pietro
\newcommand{\tc}[1]{\NoteSigned{TC}{green}{#1}}
\newcommand{\cb}[1]{\NoteSigned{CB}{brown}{#1}}
\newcommand{\cj}[1]{\NoteSigned{CJ}{purple}{#1}}
\newcommand{\sm}[1]{\NoteSigned{SM}{magenta}{#1}}

% Inline todo: Flag something in the text to be done
\newcommand{\itodo}[1]{\NoteSigned{TODO}{red}{#1}}
% Preliminary: Flag preliminary statements or results
\newcommand{\prelim}[1]{\NoteSigned{Prelim}{grey}{#1}}

% Convenient other commands
\newcommand{\sowhat}{$\rightarrow$~}


% Variant of the TODO box for addressing reviewer comments
\newcommand{\bluebox}[1]{\todo[color=blue!20!white]{#1}}

